From Benchmark to Deployment: Shift-Robust Fabric Recognition for Industrial Textile Onboarding

Automatically recognising a fabric's construction (jersey, twill, satin) is a bottleneck in textile sourcing, where incoming swatches are still typed by hand. Benchmark accuracy suggests the problem is solved, yet rarely survives deployment. On the \numClasses{}-class FabricFlow benchmark we expose three gaps that headline accuracy hides. First, a duplication audit reveals train/test leakage that inflates accuracy; we rebuild leakage-free splits that report the true difficulty. Second, on the clean data the binding failure is acquisition-source shift between catalogues, not the peripheral shortcuts one might fear: on an archive-exclusive hold-out, standard training holds 58.0\% Top-1 at a calibration error of 0.158, while a simple, architecture-agnostic central-texture recipe adds 13.5 Top-1 points and restores calibration. Third, because confusing one fabric family for another is costlier than a within-family slip, we optimise a taxonomic-severity cost: a confidence-gated routing policy auto-types confident swatches and refers only the uncertain minority to a human, sharply cutting onboarding cost. Throughout we report honest negatives: hierarchical classification, OCR fusion and zero-shot vision--language models all fail to help, yielding a concrete, calibrated, cost-aware recipe for deployable textile onboarding.

==> tables/tab_composition.tex <==
\begin{table}[t]
\centering
\footnotesize
\caption{FabricFlow composition: per-class image counts and the random-split train/val/test partition. Macro-averaged metrics are used throughout to offset the mild class imbalance.}
\label{tab:composition}
\begin{tabular}{llrrrr}
\toprule
Family & Class & Total & Train & Val & Test \\
\midrule
KNIT & Jersey & 947 & 663 & 142 & 142 \\
KNIT & Rib Knit & 954 & 668 & 143 & 143 \\
KNIT & French Terry & 976 & 683 & 146 & 147 \\
KNIT & Interlock & 417 & 292 & 62 & 63 \\
KNIT & Tricot & 290 & 203 & 44 & 43 \\
KNIT & Knit Jacquard & 666 & 466 & 100 & 100 \\
WOVEN & Plain Weave & 989 & 692 & 148 & 149 \\
WOVEN & Twill & 980 & 686 & 147 & 147 \\
WOVEN & Satin & 989 & 692 & 148 & 149 \\
WOVEN & Corduroy & 986 & 690 & 148 & 148 \\
WOVEN & Ribbed Poplin & 270 & 189 & 41 & 40 \\
WOVEN & Leno Gauze & 192 & 135 & 29 & 28 \\
WOVEN & Woven Jacquard & 660 & 462 & 99 & 99 \\
OTHERS & Mesh Lace & 1000 & 700 & 150 & 150 \\
\midrule
\multicolumn{2}{l}{Total (14 classes, 3 families)} & 10316 & 7221 & 1547 & 1548 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/tab_flat_hier_mm.tex <==
\begin{table}[t]
\centering
\footnotesize
\caption{Flat vs.\ hierarchical inference (ConvNeXt-Tiny, leakage-free split, test set).}
\label{tab:hier}
\begin{tabular}{lrrrr}
\toprule
Model & Top-1 & Top-2 & macro-F1 & ECE \\
\midrule
Flat (ConvNeXt-Tiny) & 85.48 & 94.38 & 85.23 & 0.037 \\
Hierarchical (hard cascade) & 84.34 & 90.11 & 84.01 & 0.049 \\
Hierarchical (soft marginal) & 85.12 & 92.74 & 84.78 & 0.048 \\
\textit{Oracle L1 routing} & 89.47 & 95.94 & 89.10 & 0.016 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/tab_source.tex <==
\begin{table}[t]\centering\caption{Source-aware validation.}\label{tab:source}
\textit{[pending experiments]}\end{table}

